Improving PINNs By Algebraic Inclusion of Boundary and Initial Conditions

"AI for Science" aims to solve fundamental scientific problems using AI techniques. As most physical phenomena can be described as Partial Differential Equations (PDEs) , approximating their solutions using neural networks has evolved as a central component of scientific-ML. Physics-Informed Neural Networks (PINNs) is the general method that has evolved for this task but its training is well-known to be very unstable. In this work we explore the possibility of changing the model being trained from being just a neural network to being a non-linear transformation of it - one that algebraically includes the boundary/initial conditions. This reduces the number of terms in the loss function than the standard PINN losses. We demonstrate that our modification leads to significant performance gains across a range of benchmark tasks, in various dimensions and without having to tweak the training algorithm. Our conclusions are based on conducting hundreds of experiments, in the fully unsupervised setting, over multiple linear and non-linear PDEs set to exactly solvable scenarios, which lends to a concrete measurement of our performance gains in terms of order(s) of magnitude lower fractional errors being achieved, than by standard PINNs. The code accompanying this manuscript is publicly available at, https://github.com/MorganREN/Improving-PINNs-By-Algebraic-Inclusion-of-Boundary-and-Initial-Conditions

==> Notation.tex <==

\section{Some Notation}\label{sec:note} 

\note{ 
 
The following come from the ``physics'' package except the inner-product~\\ ~\\
$\ip{\va}{\vb}, \abs{c}, \norm{\vd}, \pdv{L}{\vw}, \pdv[2]{L}{\vw}, \dv{W}{t}, \dd{x}, \rank (\mM),\tr(\mA),\Tr (\mB), \var{W}$
~\\ ~\\ 
$\relu$ is our definition
~\\ 
We have also defined the following calligraphic letters, 
$\cF, \cR, \cN, \cE, \cL, \cD$
~\\
}

\begin{center} 
\hl{This is the default highlight!}
\om{This is our customized highlight!}
\end{center} 

\note{ Everything below comes from the TMLR format \\
- which comes from this book, \url{https://github.com/goodfeli/dlbook_notation/}}

\vspace{0.5cm} 
\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\sA$ & A set\\
$\R$ & The set of real numbers \\
$\{0, 1\}$ & The set containing 0 and 1 \\
$\{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$[a, b]$ & The real interval including $a$ and $b$\\
$(a, b]$ & The real interval excluding $a$ but including $b$\\
$\sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\gG$ & A graph\\
$\parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\egroup 

~\\ ~\\
\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$a$ & A scalar (integer or real)\\
$\va$ & A vector\\
$\mA$ & A matrix\\
$\tA$ & A tensor\\
$\mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\mI$ & Identity matrix with dimensionality implied by context\\
$\ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\ra$ & A scalar random variable\\
$\rva$ & A vector-valued random variable\\
$\rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$P(\ra)$ & A probability distribution over a discrete variable\\
$p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$ f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$ f \circ g $ & Composition of the functions $f$ and $g$ \\
$f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\log x$ & Natural logarithm of $x$ \\
$\sigma(x)$ & Logistic sigmoid, $\frac{1} {1 + \exp(-x)}$ \\
$\zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\norm{\vx}_p $ & $L^p$ norm of $\vx$ \\
$\norm{\vx}$ & $L^2$ norm of $\vx$ \\
$x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
$\argmax_{\rvx \in \R^n} f$\\  
$\argmin_{\rvx \in \R^n} f$\\
$\reg, \rect,\softmax,\sigmoid,\softplus,\Var,\standarderror$\\
\end{tabular}
\egroup


